Promptly Yours? A Human Subject Study on Prompt Inference in AI-Generated Art

The emerging field of AI-generated art has witnessed the rise of prompt marketplaces, where creators can purchase, sell, or share prompts for generating unique artworks. These marketplaces often assert ownership over prompts, claiming them as intellectual property. This paper investigates whether concealed prompts sold on prompt marketplaces can be considered as secure intellectual property, given that humans and AI tools may be able to approximately infer the prompts based on publicly advertised sample images accompanying each prompt on sale. Specifically, our survey aims to assess (i) how accurately can humans infer the original prompt solely by examining an AI-generated image, with the goal of generating images similar to the original image, and (ii) the possibility of improving upon individual human and AI prompt inferences by crafting human-AI combined prompts with the help of a large language model. Although previous research has explored the use of AI and machine learning to infer (and also protect against) prompt inference, we are the first to include humans in the loop. Our findings indicate that while humans and human-AI collaborations can infer prompts and generate similar images with high accuracy, they are not as successful as using the original prompt.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}















\textbf{Fine-tuned Models.} 
Our study primarily utilized foundation and general purpose \texttt{txt2img} models for evaluating prompt inference accuracy. These models, due to their broad training across diverse data sets, offer general insights into human and AI capabilities in inferring prompts used to generate AI art. However, it is important to note that extremely fine-tuned and LoRA models, which are specialized through significantly more training on specific datasets, may exhibit different behaviors in the context of prompt inference. For example, a model fine-tuned on a specific artistic style or genre may yield images where the link between the image and its generating prompt is more obvious to humans, thereby facilitating easier inference of the prompt.

\noindent
\textbf{Expert Participants.} 
Our participant pool was primarily drawn from the general population, rather than specifically targeting individuals with expertise in AI art generation or prompt inference, which may include those with frequent engagement on platforms specialized in AI-driven artistic creation, such as Midjourney \cite{midjourney}. 
Experts in AI art generation, who have substantial experience and familiarity with AI art platforms, might possess skills and insights that could significantly influence their ability to infer prompts accurately. Their foundational understanding of how specific prompts translate into visual elements could lead to different outcomes compared to the general population.







==> framework.tex <==
\section{Framework}
\label{sec:framework}


\subsection{Text-based Classifications}
\label{sec:framework-t}




\subsection{Image-based Classifications}
\label{sec:framework-i}




\subsection{GPT4 (Blackbox) Classification}
\label{sec:framework-g}

